Revisiting Robustness in Graph Machine Learning

Many works show that node-level predictions of Graph Neural Networks (GNNs) are unrobust to small, often termed adversarial, changes to the graph structure. However, because manual inspection of a graph is difficult, it is unclear if the studied perturbations always preserve a core assumption of adversarial examples: that of unchanged semantic content. To address this problem, we introduce a more principled notion of an adversarial graph, which is aware of semantic content change. Using Contextual Stochastic Block Models (CSBMs) and real-world graphs, our results uncover: $i)$ for a majority of nodes the prevalent perturbation models include a large fraction of perturbed graphs violating the unchanged semantics assumption; $ii)$ surprisingly, all assessed GNNs show over-robustness - that is robustness beyond the point of semantic change. We find this to be a complementary phenomenon to adversarial examples and show that including the label-structure of the training graph into the inference process of GNNs significantly reduces over-robustness, while having a positive effect on test accuracy and adversarial robustness. Theoretically, leveraging our new semantics-aware notion of robustness, we prove that there is no robustness-accuracy tradeoff for inductively classifying a newly added node.

==> Camera Ready Submission_arXiv/chapters/1_introduction.tex <==
Graph Neural Networks (GNNs) are seen as state of the art for various graph learning tasks \citep{ogb1, ogb2}. However, there is strong evidence that GNNs are unrobust to changes to the underlying graph \citep{attack_nettack, attack_at_scale}. This has led to the general belief that GNNs can be easily fooled by adversarial examples and many works trying to increase the robustness of GNNs through various defenses \citep{stephan2022}. Originating from the study of deep image classifiers \citep{def_adversarial_example}, an adversarial example has been defined as a small perturbation, usually measured using an $\ell_p$-norm, which does not change the semantic content (i.e. category) of an image, but results in a different prediction. These perturbations are often termed unnoticeable relating to a human observer for whom a normal and an adversarially perturbed image are nearly indistinguishable \citep{def_adversarial_examples_2, defense_distillation}. However, compared to visual tasks, it is difficult to visually inspect (large-scale) graphs. This has led to a fundamental question:


\hspace*{\fill}\textit{What constitutes a small, semantics-preserving perturbation to a graph?}\hspace*{\fill}

The de facto standard in the literature is to measure small changes to the graph's structure %
using the $\ell_0$-pseudonorm \citep{benchmark_graph_robustness, stephan2022}. Then, the associated threat models %
restrict the total number of inserted and deleted edges globally in the graph and/or locally per node. However, if the observation of semantic content preservation for these kind of perturbation models transfers to the graph domain can be questioned: Due to the majority of low-degree nodes in real-world graphs, small $\ell_0$-norm restrictions still allow to completely remove a significant number of nodes from their original neighbourhood. Only few works introduce measures beyond $\ell_0$-norm restrictions. In particular, it was proposed to additionally use different global graph properties as a proxy for unnoticeability, such as the degree distribution \citep{attack_nettack}, degree assortativity \citep{attacks_sga}, or other homophily metrics \citep{attack_gia}. 
\begin{wrapfigure}[16]{r}{0.5\textwidth}
	\centering
	\vspace{-0.15cm}
    \includegraphics[width=0.46\textwidth]{img/starplot_final_v2.png}
	\captionof{figure}{Average degree-dependent node-classification robustness. Semantic boundary indicates when the semantics (i.e., the most likely class) of a node of a given degree changes on average. Data from CSBM graphs\protect\footnotemark. All GNNs show robustness \textit{beyond} the point of semantic change.}
	\label{fig:starplot}
\end{wrapfigure}
While these are important first steps, 
the exact relation between preserving certain graph properties and the graph's semantic content (e.g., node-categories) is unclear (see Appendix \ref{sec:app_global_graph_prop}). \footnotetext{CSBMs parametrized as outlined in Section \ref{sec:results} using $K=1.5$ and $\ell_2$\textit{-weak} attack.}For instance, one can completely rewire the graph by iteratively interchanging the endpoints of two randomly selected edges and preserve the global degree distribution%
.  As a result, current literature lacks a principled understanding of semantics-preservation in their employed notions of smallness as well as robustness studies using threat models only including provable semantics-preserving perturbations to a graph.


We bridge this gap by being the first to directly address the problem of exactly measuring (node-level) semantic content preservation in a graph under structure perturbations. Surprisingly, using Contextual Stochastic Block Models (CSBMs), this leads us to discover a novel phenomenon: GNNs show strong robustness \textit{beyond} the point of semantic change (see Figure \ref{fig:starplot}). This does \textit{not} contradict the existence of adversarial examples for the same GNNs. Related to the small degree of nodes, we find that common perturbation sets include both: graphs which are truly adversarial as well as graphs with changed semantic content. Our contributions are:
\begin{enumerate}[wide]
    \item We define a semantics-aware notion of adversarial robustness (Section \ref{sec:def_adversarial_example}) for node-level predictions. Using this, we introduce a novel concept into the graph domain: \textit{over-robustness} - that is (unwanted) robustness against admissible perturbations with changed semantic content (i.e., changed ground-truth labels). %
    \item Using CSBMs, we find: $i)$ common perturbations sets, next to truly adversarial examples, include a large fraction of graphs with changed semantic content (Section \ref{sec:extent_semantic_content_change}); $ii)$ all examined GNNs show significant \textit{over-robustness} to these graphs (Section \ref{sec:results_over_robustness}) and we observe similar patterns on real-world datasets (Section \ref{sec:over_robustness_real_graphs}). Using $\ell_0$-norm bounded adversaries on CSBM graphs, we find a considerable amount of a conventional adversarial robustness to be in fact over-robustness. 
    \item Including the known label-structure through Label Propagation (LP) \citep{correct_and_smooth} into the inference process of GNNs significantly reduces over-robustness with no negative effects on test accuracy or adversarial robustness (Section \ref{sec:results_over_robustness}) and similar behaviour on real-world graphs.
    \item Using semantic awareness, we prove the existence of a model achieving both, optimal robustness and accuracy in classifying an inductively sampled node (Section \ref{sec:robust_accuracy_tradeoff}), i.e., no robustness-accuracy tradeoff for a non-i.i.d.\ data setting.
\end{enumerate}

 










 







==> Camera Ready Submission_arXiv/chapters/2_preliminaries.tex <==
Let $n$ be the number of nodes and $d$ the feature dimension. We denote the node feature matrix $\bold{X} \in \mathbb{R}^{n \times d}$, the (symmetric) adjacency matrix $\bold{A} \in \{0,1\}^{n \times n}$, and the node labels $y \in \{0,1\}^n$ of which $y_{L} \in \{0,1\}^l$, $l \le n$ are known. We assume a graph has been sampled from a graph data generating distribution $\mathcal{D}_n$ denoted as $(\bold{X}, \bold{A}, y) \sim \mathcal{D}_n$. %
We study inductive node classification \citep{benchmark_graph_robustness}. Due to the non-i.i.d data generation%
, a node-classifier $f$ may depend its decision on the whole known graph $(\bold{X}, \bold{A}, y_L)$. %
As a result, we write $f(\bold{X}, \bold{A}, y_L)_v$ to denote the classification of a node $v$. All GNNs covered in this work are a function $f(\bold{X}, \bold{A})$ only depending on the node features $\bold{X}$ and adjacency matrix $\bold{A}$. A %
list of the used symbols and abbreviations can be found in Appendix \ref{sec:app_symbols}. 


\textbf{Label Propagation.} We use label spreading \citep{lp}, which builts a classifier $f(\bold{A}, y_{L})$ by taking the row-wise $\argmax$ of the iterate $F^t=\alpha \bold{D}^{-1/2}\bold{A}\bold{D}^{-1/2}F^{t-1}+(1-\alpha)Y$, with $\bold{D}$ being the diagonal degree matrix; $Y\in\mathbb{R}^{n \times c}$ with $Y_{ij}=1$ if $i\le l$ and $y_{L}^i=j$, otherwise $Y_{ij}=0$; and $\alpha\in[0,1]$. Similar to \citet{correct_and_smooth}, we combine LP and GNNs by replacing the zero-rows for $i > l$ in $Y$ with GNN soft-predictions, effectively forming a function $f(\bold{X}, \bold{A}, y_{L})$.

\textbf{Adversarial Robustness.} We study (inductive) evasion attacks, that is an adversary $\mathcal{A}$ can produce a perturbed graph $(\bold{\tilde{X}}, \bold{\tilde{A}})\in\mathcal{B}(\bold{X}, \bold{A})$ given the clean data $(\bold{X}, \bold{A})$ with the goal to fool a given node-classifier $f(\bold{\tilde{X}}, \bold{\tilde{A}}, y_{L})_v \ne f(\bold{X}, \bold{A}, y_{L})_v$ on nodes $v$. The perturbation set $\mathcal{B}(\bold{X}, \bold{A})$ collects all admissible perturbed graphs, defined by the threat model. We focus on direct structure attacks \citep{attack_nettack}. This means $\mathcal{A}$ can remove or add at most $\Delta \in \mathbb{N}$ edges for a target node $v$. 

\textbf{Data Model.} We leverage \textit{Contextual Stochastic Block Models} (CSBMs) \citep{csbm} to generate synthetic graphs with analytically tractable distributions. It defines edge probabilities $p$ between same-class nodes and $q$ between different-class nodes and node-features are drawn from a Gaussian mixture model. Sampling from a CSBM can be written as an iterative process over nodes $i\in [n]$: 1) Sample label $y_i \sim \text{Ber}(1/2)$ (Bernoulli distribution). 2) Sample feature vector $\bold{X}_{i,:}|y_i \sim \mathcal{N}((2y_i - 1)\mu, \sigma \bold{I})$ with $\mu \in \mathbb{R}^d$, $\sigma \in \mathbb{R}$. 3) For all $j\in[n], j < i$ sample $\bold{A}_{j,i} \sim \text{Ber}(p)$ if $y_i = y_j$ and $\bold{A}_{j,i} \sim \text{Ber}(q)$ otherwise, and set $\bold{A}_{i,j}=\bold{A}_{j,i}$. We denote this $(\bold{X}, \bold{A}, y) \sim \text{CSBM}_{n,p,q}^{\mu,\sigma^2}$. To inductively add $m$ nodes, one repeats the above process for $i=n+1, \dots, m$. %
\citet{graph_attention_retrospective} show that depending on the distance of the means $d(-\mu,\mu)$, one can separate an easy regime, where a linear classifier ignoring $\bold{A}$ can perfectly separate the data and a hard regime, defined by $d(-\mu,\mu) = K \sigma$, with $0 < K \le \mathcal{O}(\sqrt{\log n})$, where this is not possible. CSBMs are commonly used to study transductive tasks. Understanding the sampling process as an iteration extends their application to inductive node classification. For an alternative we call \textit{Contextual Barabási–Albert Model with Community Structure} (CBA) see Appendix \ref{sec:app_cba}. Appendix \ref{sec:app_graph_model_discussion} discusses the model choices.









==> Camera Ready Submission_arXiv/chapters/3_revisting_adversarial_pert.tex <==
Given a clean graph $(\bold{X}, \bold{A}, y_{L})$ and target node $v$. The perturbation set $\mathcal{B}(\bold{X}, \bold{A})$ comprises all possible (perturbed) graphs $(\tilde{\bold{X}}, \tilde{\bold{A}})$, which can be chosen by an adversary $\mathcal{A}$, with the goal to change the prediction of a node classifier $f$, i.e., $f(\tilde{\bold{X}}, \tilde{\bold{A}}, y_L)_v \ne f(\bold{X}, \bold{A}, y_L)_v$. The prevalent works implicitly assume that every $(\tilde{\bold{X}}, \tilde{\bold{A}}) \in \mathcal{B}(\bold{X}, \bold{A})$ preserves the node-level semantic content of the clean graph, i.e., the original ground-truth label of $v$. %
If we would have an oracle $\Omega$, which tells us the semantic content the known graph encodes about $v$, this assumption can be made explicit by writing $\Omega(\tilde{\bold{X}}, \tilde{\bold{A}}, y_L)_v = \Omega(\bold{X}, \bold{A}, y_L)_v$. %
Usually, we do not have access to such an oracle. However, we can try to model its behaviour by introducing a reference or base node classifier $g$. Then, the idea is to use $g$ to indicate semantic content change and thereby, define the semantic boundary (see Figure \ref{fig:starplot}). Exemplary, $g$ could be derived from knowledge about the data generating process. We do so in Section \ref{sec:bayes_classifier} and \ref{sec:results}, where we use the (Bayes) optimal classifier for CSBMs as $g$. Note that labels themselves are often generated following a base classifier. Exemplary, this can be humans labelling selected nodes in a graph to generate a dataset for (semi-) supervised learning. %
Using a reference classifier $g$ as a proxy for semantic content enables us to make a refined definition of an adversarial graph, which makes the unchanged-semantics assumption explicit:
\begin{definition}\label{def:adversarial_perturbation}
Let $f$ be a node classifier and $g$ a reference node classifier. Then the perturbed graph $(\Tilde{\bold{X}}, \Tilde{\bold{A}}) \in \mathcal{B}(\bold{X}, \bold{A})$ chosen by an adversary $\mathcal{A}$ is said to be adversarial for $f$ at node $v$ w.r.t.\ the reference classifier $g$ if the following conditions are satisfied:
\begin{align*}
    \text{i.} \quad & %
    f(\bold{X}, \bold{A}, y_\text{L})_v = g(\bold{X}, \bold{A}, y_\text{L})_v \qquad \text{(correct clean prediction)}
    \\
    \text{ii.} \quad  & %
    g(\Tilde{\bold{X}}, \Tilde{\bold{A}}, y_\text{L})_v = g(\bold{X}, \bold{A}, y_\text{L})_v \qquad \text{(perturbation preserves semantics)} 
    \\
    \text{iii.} \quad  & %
    f(\bold{\tilde{X}}, \bold{\tilde{A}}, y_\text{L})_v \ne g(\bold{X}, \bold{A}, y_\text{L})_v \qquad \text{(node classifier changes prediction)}
\end{align*}
\end{definition}
Definition \ref{def:adversarial_perturbation} says that a perturbed graph $(\tilde{\bold{X}}, \tilde{\bold{A}}) \in \mathcal{B}(\bold{X}, \bold{A})$ only then is adversarial, if $(\tilde{\bold{X}}, \tilde{\bold{A}})$ does not only change the prediction of the node classifier $f$ $(iii)$, but also lets the original label unchanged $(ii)$. The first constraint $(i)$ stems from the fact that if $f$ and $g$ disagree on the clean graph at node $v$ this should represent a case of misclassification captured by standard error metrics such as accuracy.

\citet{revisiting_adv_risk} use the concept of a reference classifier to, in similar spirit, define semantics-aware adversarial perturbations for i.i.d.\ data, with a focus on the image domain. However, what has not been considered is that the reference classifier allows us to characterize the exact opposite behaviour of an adversarial example: if a classifier $f$ does not change its prediction for a perturbed graph $(\tilde{\bold{X}}, \tilde{\bold{A}})$ even though the semantic content has changed. As this would mean that $f$ is robust beyond the point of semantic change, we call this behaviour \textit{over-robustness}:
\begin{definition}\label{def:over_robustness}
Let $f$ be a node classifier and $g$ a reference node classifier. Then the perturbed graph $(\Tilde{\bold{X}}, \Tilde{\bold{A}}) \in \mathcal{B}(\bold{X}, \bold{A})$ chosen by an adversary $\mathcal{A}$ is said to be an over-robust example for $f$ at node $v$ w.r.t.\ the reference classifier $g$ if the following conditions are satisfied:
\begin{align*}
    \text{i.} \quad & f(\bold{X}, \bold{A}, y_\text{L})_v = g(\bold{X}, \bold{A}, y_\text{L})_v \qquad \text{(correct clean prediction)}\\
    \text{ii.} \quad & g(\Tilde{\bold{X}}, \Tilde{\bold{A}}, y_\text{L})_v \ne g(\bold{X}, \bold{A}, y_\text{L})_v \qquad \text{(perturbation changes semantics)}  \\
    \text{iii.} \quad & f(\bold{\tilde{X}}, \bold{\tilde{A}}, y_\text{L})_v = g(\bold{X}, \bold{A}, y_\text{L})_v \qquad \text{(node classifier stays unchanged)}
\end{align*}
If there exists such an over-robust example, we call $f$ over-robust at node $v$ w.r.t.\ $g$.
\end{definition}
Definition \ref{def:over_robustness} is of particular interest in the graph domain, where perturbation sets $\mathcal{B}(\bold{X}, \bold{A})$ often include graphs $(\Tilde{\bold{X}}, \Tilde{\bold{A}})$, which allow significant changes to the neighbourhood structure of $v$%
, but do not allow easy manual content inspection. Indeed, Section \ref{sec:results} shows that all assessed GNNs are over-robust for common choices of $\mathcal{B}(\bold{X}, \bold{A})$ for many test nodes $v$ in CSBM graphs. A similar phenomenon for image data has been discussed by \citet{invariance_based_adv_examples}. %

\begin{wrapfigure}[16]{r}{0.43\textwidth}
    \vspace{-0.65cm}
    \centering
    \begin{subfigure}[b]{0.185\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{img/concept_basic_v3.png}
         \caption{}
         \label{fig:concept_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.185\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{img/concept_2_v2.png}
         \caption{}
         \label{fig:concept_2}
     \end{subfigure}
    \caption{a) Decision boundary of classifier $f$ follows a base classifier $g$ except for the dotted line. b) Finite perturbation sets $\mathcal{B}( \cdot )$ intersect only from one side with the dashed area. Over- and adversarial robustness are needed to characterize robustness.}
    \label{fig:concept}
\end{wrapfigure}
Now, let us contrast over- to adversarial robustness.
In Figure \ref{fig:concept_1} the decision boundary  
of a classifier $f$ follows the one of a base classifier $g$ except for the dotted line%
. %
The dashed area between $f$ and $g$ is a region of over-robustness for the blue class and %
of adversarial examples for the red class. %
In practice, %
the extent of the perturbation sets $\mathcal{B}( \cdot )$ is bounded. As a result, using adversarial examples, it is only possible to measure the right boundary of the dashed area (see Figure \ref{fig:concept_2}). %
The concept of over-robustness allows us to additionally measure the left boundary and hence, provides a more complete picture of the robustness of $f$. Note that the blue points, using conventional adversarial robustness, are judged robust in the whole of $\mathcal{B}(\cdot)$ even though their true class changed. Semantic-aware adversarial robustness 
allows to (correctly) cut off $\mathcal{B}(\cdot)$ at the decision boundary of $g$.

Contrary to Figure \ref{fig:concept_1}, a region of over-robust examples cannot always be identified as a region of adversarial examples for different data points. Denote $\mathcal{G}$\,$=$\,$(\bold{X}, \bold{A})$ and collect all over-robust examples in a set $\mathcal{B}_{O}(\mathcal{G},v) \subset \mathcal{B}(\mathcal{G})$ and adversarial examples in a set $\mathcal{B}_{A}(\mathcal{G},v) \subset \mathcal{B}(\mathcal{G})$. Note that it follows from Definition \ref{def:adversarial_perturbation} and \ref{def:over_robustness} that %
$\mathcal{B}_{O}(\mathcal{G},v) \cap \mathcal{B}_{A}(\mathcal{G},v) = \emptyset$. 
Now, we find that in general, for a given over-robust example $\tilde{\mathcal{G}}\in\mathcal{B}(\mathcal{G})$ one can't always find a corresponding clean graph $\mathcal{G}' \ne \mathcal{G}$ not in $\mathcal{B}(\mathcal{G})$ for which $\tilde{\mathcal{G}}$ is an adversarial example. It suffices to look at the case of $f$ being constant:
\begin{proposition} \label{corollary:constant_f}
Given $f$ is a constant classifier, then $\mathcal{B}_{A}(\mathcal{G},v)$ is empty for every possible graph $\mathcal{G}$.
\end{proposition}
This follows as $f$ can never fulfill both, item $(i)$ and item $(iii)$ in Definition \ref{def:adversarial_perturbation}. However, over-robust examples for $f$ may exists. Every example in $\mathcal{B}(\mathcal{G})$ will be over-robust, for which $g$ changes its label for node $v$. This also shows that  \textit{over-robustness} can differentiate two classifiers, which have the same adversarial robustness, but one has learned a better decision boundary, while the other has not. 
We further develop other interesting conceptual cases in Appendix \ref{sec:app_over_vs_adversarial}.




==> Camera Ready Submission_arXiv/chapters/4_bayes_classifier.tex <==
In the following, we derive a Bayes optimal classifier to use as a reference classifier $g$. Using the Bayes decision rule as $g$ is a natural choice, because, as shown below, it provides us with the information, if another class is now more likely based on the true data generating distribution and hence, is the closest we can get to a semantic content returning oracle $\Omega$ (see Section \ref{sec:def_adversarial_example}). 

Assume that we want to learn an inductive node-classifier $f$ on a given, fully labeled graph $(\bold{X}, \bold{A}, y) \sim \mathcal{D}_n$ with $n$ nodes. We will focus on the most simple case of classifying an inductively sampled node. We denote the conditional distribution over graphs with an inductively added node as $\mathcal{D}(\bold{X}, \bold{A}, y)$. Then, the target node $v$ corresponds to the newly sampled, $n+1$-th node.  
How well our classifier $f$ generalizes to the newly added node is captured by the expected $0/1$-loss of $f$:
\begin{equation} \label{eq:expected_loss_1_node}
    \underset{(\bold{X}', \bold{A}', y')\sim \mathcal{D}(\bold{X}, \bold{A}, y)}{\mathbb{E}}[\ell_{0/1}(y_v', f(\bold{X}', \bold{A}', y)_v]
\end{equation}
To derive Bayes optimality, we have to find an optimal classifier $f^*$ for $v$, depending on $(\bold{X}', \bold{A}', y)$, minimizing (\ref{eq:expected_loss_1_node}). The following theorem shows that, similar to inductive classification for i.i.d. data, $f^*$ should choose the most likely class based on the seen data (Proof in Appendix \ref{sec:proof_bayes}): %


\begin{theorem}\label{theorem:bayes_classifier}
The Bayes optimal classifier, minimizing the expected $0/1$-loss (\ref{eq:expected_loss_1_node}), is 
$f^*(\bold{X}', \bold{A}', y)_v = \arg\max_{\hat{y} \in \{0,1\}} \mathbb{P}[y'_v = \hat{y} | \bold{X}', \bold{A}',y]$.
\end{theorem}

\subsection{Robustness-Accuracy Tradeoff} \label{sec:robust_accuracy_tradeoff}

We show that given a Bayes optimal reference classifier $g$, our robustness notions (Definition \ref{def:adversarial_perturbation} and \ref{def:over_robustness}) imply that optimal robustness, i.e., the non-existence of adversarial and over-robust examples for $f$, is possible while preserving good generalization in the sense of (\ref{eq:expected_loss_1_node}). Our argumentation for the non-i.i.d.\ graph data case takes inspiration from \citet{revisiting_adv_risk}'s study for i.i.d.\ data. In the following, we assume we are given a graph $\mathcal{G}'$ sampled from $\mathcal{D}(\mathcal{G}, y)$, where $\mathcal{G}=(\bold{X}, \bold{A})$ represents a fully labeled training graph with $n$ nodes and labels $y$. Let $v$ refer to the $n+1$-th (inductively added) node. First, observe from Definition \ref{def:adversarial_perturbation} that a graph $\tilde{\mathcal{G}}' \in \mathcal{B}(\mathcal{G}')$ is an adversarial example, iff $g(\tilde{\mathcal{G}}', y)_v = g(\mathcal{G}', y)_v$ and $\ell_{0/1}(f(\tilde{\mathcal{G}}', y)_v, g(\mathcal{G}', y)_v) - \ell_{0/1}(f(\mathcal{G}', y)_v, g(\mathcal{G}', y)_v) = 1$. In analogy to the generalization error (\ref{eq:expected_loss_1_node}), we define the adversarial generalization error:

\begin{definition}
Let $f$ be a node classifier and $g$ a reference node classifier. Assume $\mathcal{G}'$ is itself in $ \mathcal{B}(\mathcal{G}')$. Then the expected adversarial $0/1$-loss for an inductively added target node $v$ is defined as the probability that a conditionally sampled graph can be adversarially perturbed:
\begin{align} \label{eq:expected_adversarial_loss}
    \underset{(\mathcal{G}', y')\sim \mathcal{D}(\mathcal{G}, y)}{\mathbb{E}}\Bigg[
    \max_{\substack{\tilde{\mathcal{G}}' \in \mathcal{B}(\mathcal{G}') \\ g(\tilde{\mathcal{G}}', y)_{v} = g(\mathcal{G}', y)_{v}}}
     \left\{\ell_{0/1}(f(\tilde{\mathcal{G}}', y)_{v}, g(\mathcal{G}', y)_{v}) 
     - \ell_{0/1}(f(\mathcal{G}', y)_{v}, g(\mathcal{G}', y)_{v})\right\}\Bigg]
\end{align}
\end{definition}


From Definition \ref{def:over_robustness} it follows that a graph $\tilde{\mathcal{G}}' \in \mathcal{B}(\mathcal{G})$ is an over-robust example, iff $f(\tilde{\mathcal{G}}', y)_v = f(\mathcal{G}', y)_v$ and $\ell_{0/1}(g(\tilde{\mathcal{G}}', y)_v, f(\mathcal{G}', y)_v) - \ell_{0/1}(g(\mathcal{G}', y)_v, f(\mathcal{G}', y)_v) = 1$. Thus, we define:

\begin{definition}
Let $f$ be a node classifier and $g$ a reference node classifier. Assume $\mathcal{G}'$ is itself in $\mathcal{B}(\mathcal{G}')$. Then the expected over-robust $0/1$-loss for an inductively added target node $v$ is defined as the probability that a conditionally sampled graph can be perturbed to be an over-robust example:
\begin{align} \label{eq:expected_robust_loss}
    \underset{(\mathcal{G}', y')\sim \mathcal{D}(\mathcal{G}, y)}{\mathbb{E}}\Bigg[
    \max_{\substack{\tilde{\mathcal{G}}' \in \mathcal{B}(\mathcal{G}') \\ f(\tilde{\mathcal{G}}', y)_{v} = f(\mathcal{G}', y)_{v}}}
     \left\{\ell_{0/1}(g(\tilde{\mathcal{G}}', y)_v, f(\mathcal{G}', y)_v) 
     - \ell_{0/1}(g(\mathcal{G}', y)_v, f(\mathcal{G}', y)_v)\right\}\Bigg]
\end{align}
\end{definition}


We denote the expected adversarial $0/1$-loss as $\mathscr{L}_{\mathcal{G}, y}^{adv}(f,g)_v$ and the expected over-robust $0/1$-loss as $\mathscr{L}_{\mathcal{G}, y}^{over}(f,g)_v$. Minimizing only one of the robust objectives and disregarding the standard loss (\ref{eq:expected_loss_1_node}), may not yield a sensible classifier. Exemplary, the adversarial loss (\ref{eq:expected_adversarial_loss}) achieves its minimal value of $0$ for a constant classifier. %
Therefore, we collect them in an overall expected robustness loss term:
\begin{equation}\label{eq:real_expected_robust_loss}
    \mathscr{L}_{\mathcal{G}, y}^{rob}(f,g)_v = \lambda_1 \mathscr{L}_{\mathcal{G}, y}^{adv}(f,g)_v + \lambda_2 \mathscr{L}_{\mathcal{G}, y}^{over}(f,g)_v
\end{equation}
where $\lambda_1 \ge 0$ and $\lambda_2 \ge 0$ define how much weight we give to the adversarial and the over-robust loss. Now, we want to find a node-classifier $f$ with small robust and standard loss. Denoting the expected $0/1$-loss (\ref{eq:expected_loss_1_node}) as $\mathscr{L}_{\mathcal{G}, y}(f)_v$, this leads us to optimize the following objective:
\begin{equation}\label{eq:combined_loss}
    \argmin_{f \in \mathcal{H}} \mathscr{L}_{\mathcal{G}, y}(f)_v + \lambda \mathscr{L}_{\mathcal{G}, y}^{rob}(f,g)_v
\end{equation}
where $\lambda \ge 0$ defines a tradeoff between standard accuracy and robustness and $\mathcal{H}$ represent a set of admissible functions, e.g. defined by a chosen class of GNNs. Now, the following holds:

\begin{theorem} \label{theorem:tradeoff}
Assume a set of admissible functions $\mathcal{H}$, which includes a Bayes optimal classifier $f^*_{Bayes}$ and let the reference classifier $g$ be itself a Bayes optimal classifier. Then, any minimizer $f^* \in \mathcal{H}$ of (\ref{eq:combined_loss}) is a Bayes optimal classifier. 
\end{theorem}

Proof see Appendix \ref{sec:proof_theorem2}. Theorem \ref{theorem:tradeoff} implies that minimizing both, the standard and robust loss for any $\lambda \ge 0$, always yields a Bayes optimal classifier. Therefore, optimizing for robustness does not tradeoff accuracy of the found classifier by (\ref{eq:combined_loss}) and hence, establishes that classifying an inductively sampled node does not suffer from a robustness-accuracy tradeoff. %
Theorem \ref{theorem:tradeoff} raises the important question if common GNNs define function classes $\mathcal{H}_{GNN}$ expressive enough to represent a Bayes classifier for (\ref{eq:expected_loss_1_node}) and hence, can achieve optimal robustness. Theorem \ref{theorem:min_robust_loss} in Appendix \ref{sec:proof_theorem3} shows that only being a minimizer for the robust loss $\mathscr{L}_{\mathcal{G}, y}^{rob}(f,g)_v$ does not imply good generalization.




==> Camera Ready Submission_arXiv/chapters/5_results.tex <==
\begin{wraptable}[17]{r}{0.2\textwidth}
\vspace{-0.8cm}
\tabcolsep=0.09cm
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}\\
\multicolumn{3}{c}{\textbf{Accuracy (Bayes)}} \\
\textbf{K} & $\bold{X}$ & $(\bold{X}, \bold{A})$ \\ \toprule  %
0.1 & 50.8\% & 89.7\% \\  %
0.5 & 59.0\% & 90.3\%\\ 
1.0 & 68.4\% & 91.7\%\\ 
1.5 & 76.5\% & 93.1\%\\ 
2.0 & 83.4\% & 94.7\%\\ 
3.0 & 92.6\% & 97.4\%\\ 
4.0 & 97.5\% & 99.0\% \\ 
5.0 & 99.3\% & 99.8\%\\ 
\end{tabular}
}
\caption{Mean accuracy of the Bayes optimal classifier on test nodes $v$ with $(\bold{X}, \bold{A})$ and without ($\bold{X}$) structure information.} %
\label{tab:bc_features_separability}
\end{wraptable} 

Using Contextual Stochastic Block Models (CSBMs) we measure the extent of semantic content violations in common threat models (Section \ref{sec:extent_semantic_content_change}). Then, we study over-robustness in CSBMs (Section \ref{sec:results_over_robustness}) and real-world graphs (Section \ref{sec:over_robustness_real_graphs}). In CSBMs, we use the Bayes optimal classifier (Theorem \ref{theorem:bayes_classifier}), denoted $g$, to measure semantic change. %
The robustness of the Bayes classifier defines the maximal meaningful robustness achievable %
(see Section \ref{sec:def_adversarial_example}). For results using the Contextual Barabási–Albert Model with Community Structure (CBA), we refer to Appendix \ref{sec:results_cba}.

\textbf{Experimental Setup.} We sample training graphs with $n$\,$=$\,$1000$ nodes from a $\text{CSBM}_{n,p,q}^{\mu,\sigma^2}$ in the hard regime (Section \ref{sec:preliminaries}). Each element of the class mean vector $\mu \in \mathbb{R}^d$ is set to $K\sigma/2\sqrt{d}$, resulting in a distance between the class means of $K\sigma$. We set $\sigma=1$ and vary $K$ from close to \textit{no} discriminative features $K$\,$=$\,$0.1$ to making structure information \textit{unnecessary} $K$\,$=$\,$5$ (see Table \ref{tab:bc_features_separability}). We choose $p$\,$=$\,$0.63$\% and $q$\,$=$\,$0.15$\% resulting in the expected number of same-class and different-class edges for a given node to fit CORA \citep{cora}. Following \citet{graph_attention_retrospective}, we set $d$\,$=$\,$\lfloor n/\ln^2(n) \rceil$\,$=$\,$21$. We use an $80$\%$/20$\% train/validation split on the nodes. As usual in the inductive setting, we remove the validation nodes from the graph during training. At test time, we inductively sample $1000$ times an additional node conditioned on the training graph. For each $K$, we sample $10$ different training graphs. 

\textbf{Models and Attacks.} We study a wide range of popular GNN architectures: Graph Convolutional Networks (GCN) \citep{gcn}, Simplified Graph Convolutions (SGC) \citep{sgc}, Graph Attention Networks (GAT) \citep{gat}, GATv2 \citep{gatv2}, APPNP \citep{appnp}, and GraphSAGE \citep{graphsage}. Furthermore, we study a simple Multi-Layer Perceptron (MLP) and Label Propagation
(LP) \citep{lp}. The combination of a model with LP \citep{correct_and_smooth} is denoted by \textit{Model+LP} (see Section \ref{sec:preliminaries}). To find adversarial examples, we employ the established attacks \textit{Nettack} \citep{attack_nettack}, \textit{DICE} (random addition of different-class edges) \citep{attack_dice}, \textit{GR-BCD}~\citep{attack_at_scale} and \textit{SGA} \citep{attack_at_scale}. Furthermore, we employ $\ell_2$\textit{-strong}: Connect to the most distant different-class nodes in feature space using $\ell_2$-norm. 
To find over-robust examples, we use a "weak" attack, which we call \textit{$\ell_2$-weak}: Connect to the closest different-class nodes in $\ell_2$-norm. Theorem \ref{theorem:app_proof_optimal_attack} in Appendix \ref{sec:app_proof_optimal_attack} shows that a strategy to change, with least structure changes, the true most likely class on CSBMs, i.e., an "optimal attack" against the Bayes classifier $g$, is given by (arbitrarily) disconnecting same-class edges and adding different-class edges to the target node. Therefore, the attacks \textit{DICE}, $\ell_2$\textit{-strong}, and $\ell_2$\textit{-weak} have the same effect on the semantic content of a graph. We investigate perturbation sets $\mathcal{B}_{\Delta}( \cdot )$ with local budgets $\Delta$ from $1$ up to the degree (deg) of a node\,+\,2, similarly to \citet{attack_nettack}. Further details, including the hyperparameter settings can be found in Appendix \ref{sec:app_experiment_details}. 

\textbf{Robustness Metrics}. To analyse the robustness of varying models across different graphs, we need to develop comparable metrics summarizing the robustness properties of a model $f$ on a given graph. First, to correct for the different degrees of nodes, we measure the adversarial robustness of $f$ (w.r.t.\ $g$) at node $v$ relative to $v$'s degree and average over all test nodes $V'$\footnote{Excluding degree $0$ nodes. This is one limitation of this metric, however, these are very rare in the generated CSBM graphs and non-existing in common benchmark datasets such as CORA.}:
\begin{equation}\label{eq:metric_degree_corrected_robustness}
    R(f,g) = \frac{1}{|V'|}\sum\nolimits_{v \in V'}{\frac{\text{Robustness}(f, g, v)}{\text{deg}(v)}}
\end{equation}
where $g$ represents the Bayes classifier and hence, $\text{Robustness}(f, g, v)$ refers to the (minimal) number of semantics-aware structure changes $f$ is robust against (Definition \ref{def:adversarial_perturbation}). Exemplary, $R(f,g)=0.5$ would mean that on average, node predictions are robust against changing $50$\% of the neighbourhood structure. Using the true labels $y$ instead of a reference classifier $g$ in (\ref{eq:metric_degree_corrected_robustness}), yields the conventional (degree-corrected) adversarial robustness, unaware of semantic change, which we denote $R(f):=R(f,y)$. To measure \textbf{over-robustness}, we measure the fraction of conventional adversarial robustness $R(f)$, which cannot be explained by semantic-preserving robustness $R(f,g)$: $R^{over} = 1 - R(f,g) / R(f)$. Exemplary, $R^{over}=0.2$ means that $20$\% of the measured robustness is robustness beyond semantic change. In Appendix \ref{sec:app_metrics} we present a metric for semantic-aware adversarial robustness and how to calculate an overall robustness measure using the harmonic mean.

\subsection{Extent of Semantic Content Change in Common Perturbation Models} \label{sec:extent_semantic_content_change}

\begin{wraptable}[17]{r}{0.5\textwidth}
\vspace{-0.8cm}
\tabcolsep=0.08cm
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{lrrrrrrrr}\\
\textbf{Threat}& \multicolumn{8}{c}{\textbf{K}} \\
\textbf{Models} & $0.1$ & $0.5$& $1.0$& $1.5$& $2.0$& $3.0$& $4.0$& $5.0$\\ \toprule 
$\mathcal{B}_1(\cdot)$ & 14.3 &  11.2 &  9.1 &  6.8 &  4.4 &  1.9 &  0.8 &  0.2  \\  %
$\mathcal{B}_2(\cdot)$ &  35.9 &  31.2 &  25.7 &  19.8 &  14.1 &  6.2 &  2.2 &  0.7  \\ 
$\mathcal{B}_3(\cdot)$ &  58.5 &  53.8 &  46.8 &  38.2 &  28.8 &  14.3 &  5.1 &  1.7  \\ 
$\mathcal{B}_4(\cdot)$ & 76.5 &  73.0 &  66.6 &  58.1 &  47.0 &  25.7 &  9.8 &  3.4  \\ 
$\mathcal{B}_{\text{deg}}(\cdot)$ &  75.7 &  60.0 &  55.4 &  49.1 &  39.6 &  21.9 &  9.0 &  3.2\\ 
$\mathcal{B}_{\text{deg+2}}(\cdot)$ & 100\, &  100\, &  99.4 &  92.9 &  80.5 &  51.7 &  24.8 &  9.1  \\ 
\end{tabular}
}
\caption{Percentage (\%) of test nodes for which perturbed graphs in $\mathcal{B}_\Delta(\cdot)$ violate semantic content preservation. Calculated by connecting $\Delta$ different class nodes ($\ell_2$-weak) to every target node. For $K$$\ge$$4.0$ structure is not necessary for good generalization (Table \ref{tab:bc_features_separability}). Results using other attacks are similar (see Appendix \ref{sec:app_results_semantic_change}). Standard deviations are insignificant and hence, omitted.} 
\label{tab:prevalence_semantic_violated}
\end{wraptable}
We investigate how prevalent perturbed graphs with changed semantic content are for common perturbation model choices. We denote the perturbation set allowing a local budget of $\Delta$ edge perturbations as $\mathcal{B}_\Delta(\cdot)$. Table \ref{tab:prevalence_semantic_violated} shows the fraction of test nodes, for which we find perturbed graphs in $\mathcal{B}_\Delta(\cdot)$ with changed ground truth labels. Surprisingly, even for very modest budgets, if structure matters ($K \le 3$), this fraction is significant. Exemplary, for $K$$=$$1.0$ and $\mathcal{B}_\text{deg+2}(\cdot)$, we
find perturbed graphs with changed semantic content for 99.4\% of the target nodes. This establishes for CSBMs, a \textit{negative} answer to a question formulated in the introduction: \textit{If structure matters, does completely reconnecting a node preserve its semantic content?} Similar to CSBMs, nodes in real-world graphs have mainly low-degree (Figure \ref{fig:degree_distribution_cora_csbm} in Appendix \ref{sec:app_results_degree_distr}). This provides evidence that similar conclusion could be drawn for certain real-world graphs. The examined $\mathcal{B}_\Delta(\cdot)$ subsume all threat models against edge-perturbations employing the $\ell_0$-norm to measure small changes to the graph's structure, as we investigate the lowest choices of local budgets possible\footnote{Global budgets again result in local edge-perturbations, however, now commonly allowing for way stronger perturbations than $\mathcal{B}_\text{deg+2}(\cdot)$ to individual nodes. The number of allowed perturbation is usually set to a small one- or two-digit percentage of the total number of edges in the graph. For CORA with $5278$ edges, a relative budget of $5$\% leads to a budget of $263$ edge-changes, which can be distributed in the graph without restriction.} and for these already find a large percentage of perturbed graphs, violating the semantics-preservation assumption. %

Values in Table \ref{tab:prevalence_semantic_violated} are lower bounds on the prevalence of graphs in $\mathcal{B}_\Delta(\cdot)$ with changed semantic content. We calculate these values by connecting $\Delta$ different-class nodes ($\ell_2$-weak) to every target node and hence, the constructed perturbed graphs $\tilde{\mathcal{G}}$ are at the boundary of $\mathcal{B}_\Delta(\cdot)$. Then, we count how many $\tilde{\mathcal{G}}$ have changed their true most likely class using the Bayes classifier $g$. Thus, exemplary, if a classifier $f$ is robust against $\mathcal{B}_3(\cdot)$ for CSBMs with $K$$=$$1.0$, $f$ classifies the found graphs at the boundary of $\mathcal{B}_3(\cdot)$ wrong in $47$\% of cases. Therefore, $f$ shows high \textbf{over-robustness} $R^{over}$.   

\subsection{Over-Robustness of Graph Neural Networks} \label{sec:results_over_robustness}

\begin{figure}[t]
    \centering
    \hspace{-1.15cm}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=1.17\textwidth]{img/results/overrobust_l2weak_deg+0_vRebutal2.png}
         \caption{Local Budget $\Delta$\textbf: Degree of Node }
         \label{fig:over_robustness_deg}
    \end{subfigure}
    \hspace{-1.20cm}
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=1.17\textwidth]{img/results/overrobust_l2weak_vRebutal.png}
         \caption{No Budget Restriction.}
         \label{fig:over_robustness}
     \end{subfigure}
    \caption{Fraction of Robustness beyond Semantic Change (Attack: $\ell_2$-weak; Plot with Standard Error). (a) A large part of the measured robustness against $\mathcal{B}_{\text{deg}}(\cdot)$ can be attributed to over-robustness. (b) Applying $\ell_2$-weak without budget restriction until it changes a classifiers prediction. Note that over-robustness can be significantly reduced by label propagation and for (b) that some over-robust models, especially for high $K$, show high adversarial robustness (Appendix \ref{sec:app_results_adversarial_robustness}).}
    \vspace{-0.4cm}
\end{figure}

Section \ref{sec:extent_semantic_content_change} establishes the \textbf{existence} of perturbed graphs with changed semantic content in common threat models. Now, we examine how much of the measured robustness of common GNNs can actually be attributed to over-robustness ($R^{over}$), i.e., to robustness beyond semantic change. As a qualitative example, we study a local budget of the degree of the target nodes $\mathcal{B}_{\text{deg}}( \cdot )$, results on other perturbation sets can be found in Appendix \ref{sec:app_over_robustness_otherB}. Figure \ref{fig:over_robustness_deg} shows the over-robustness of GNNs when attacking their classification of inductively added nodes. For $K\le3$ the graph structure is relevant in the prediction (see Table \ref{tab:bc_features_separability}). We find that in this regime, a significant amount of the measured robustness of \textbf{all} GNNs can be attributed to \textbf{over-robustness}. Exemplary, $30.3$\% of the conventional adversarial robustness measurement of a GCN for $K=0.5$ turns out to be over-robustness. LP achieves the lowest $R^{over}$ and $R^{over}$ \textbf{significantly reduces} when it is applied on top of a GNN. Exemplary, GCN+LP for $K=0.5$ drops to $R^{over}=20.9$\%. Adding LP does \textbf{not} decrease test-accuracy (Appendix \ref{sec:app_test_accuracy}) and often \textbf{increases} adversarial robustness as long as structure matters (see Figure \ref{fig:app_nettack_adv_robustness_deg+0} in Appendix \ref{sec:app_results_adversarial_robustness_nettack}). 

An MLP achieves maximal robustness. Thus, for attacks choosing perturbations independent of the attacked model, it provides an upper bound on the measurable over-robustness for a particular node, as the complete budget $\Delta$ will be exhausted without flipping an MLP's prediction. Exemplary, we measure $43$\% over-robustness for $K$\,$=$\,$0.1$ using $\ell_2$-weak. This means that for a perfectly robust classifier against $\mathcal{B}_{\text{deg}}( \cdot )$ for CSBM graphs with $K$\,$=$\,$0.1$, $43$\% of measured conventional adversarial robustness against $\ell_2$-weak is undesirable over-robustness. Note that all GNNs are \textbf{close} to this upper bound. Stronger attacks such as Nettack or GR-BCD still show that a significant part of the measured robustness is over-robustness (see Appendix \ref{sec:app_results_over_robustness}). Exemplary, Nettack performs strongest against SGC and GCN. However, for a GCN at $K=0.5$, still $11.4$\% of the measured robustness is in fact over-robustness. An MLP for Nettack for $K=2$ still shows $19.2$\% $R^{over}$, indicating that we can expect a model robust against Nettack in $\mathcal{B}_{\text{deg}}(\cdot)$ to have high $R^{over}$. For bounded perturbation sets $\mathcal{B}_\Delta(\cdot)$, maximal over-robustness necessarily decreases if $K$ increases, as the more informative features are, the more structure changes it takes to change the semantic content (i.e., the Bayes decision). Thus, less graphs in $\mathcal{B}_\Delta(\cdot)$ have changed semantics (also see Table \ref{tab:prevalence_semantic_violated}). 

As a \textbf{positive take-away} for robustness measurements on real-world graphs, we find that if the attack is strong enough, the robustness rankings derived from conventional adversarial robustness are \textbf{consistent} with using semantic-aware adversarial robustness (Appendix \ref{sec:app_results_adversarial_robustness_nettack} and \ref{sec:app_results_adversarial_robustness_grbcd}). However, if the attack is weak, semantic-awareness can \textbf{significantly} change robustness rankings (Appendix \ref{sec:app_results_adversarial_robustness_dice} and \ref{sec:app_results_adversarial_robustness_sga}). For high $K$, some GNNs show high (semantics-aware) adversarial robustness (Appendix \ref{sec:app_results_adversarial_robustness_nettack}) additional to high $R^{over}$. Interestingly, if structure matters, the best harmonic mean robustness is in general achieved by MLP+LP (Appendix \ref{sec:app_results_adversarial_robustness}), which also has the best non-trivial adversarial robustness, while achieving competitive test-accuracies. For Figure \ref{fig:over_robustness}, we apply $\ell_2$-weak without budget restriction until it changes a model's prediction. As a result, we find that all GNNs (but not LP) have extensive areas of over-robustness in input space (compare to Figure \ref{fig:app_concept} in Appendix \ref{sec:app_over_vs_adversarial}).


\subsubsection{Over-Robustness on Real-World Graphs} \label{sec:over_robustness_real_graphs}

Table \ref{tab:prevalence_semantic_violated} shows that only a few perturbations can change the semantic-content a graph encodes about a target node. Additionally, if structure matters ($K\le3$), the Bayes decision on CSBMs changes on average after at most changing as many edges as the target node's degree. This is visualized in Figure \ref{fig:starplot} measured for $K$$=$$1.5$ and for other $K$ in Figure \ref{fig:app_avg_robustness_bayes}  
in Appendix \ref{sec:app_avg_robustness_bayes}. It is challenging to derive a reference classifier for real-world datasets and hence, directly measure over-robustness. However, 
we can investigate the degree-dependent robustness of GNNs and see if we similarly find high robustness beyond the degree of nodes. Figure \ref{fig:over_robustness_cora_ml} 
shows that a majority of test node predictions of a GCN on (inductive) Cora-ML \citep{cora_ml} are robust beyond their degree, by several multiples. The median robustness for degree $1$ nodes, lies at over $10$ structure changes.
Figure \ref{sec:app_boxplot_csbm_vs_coraml} 
\begin{wrapfigure}[11]{r}{0.34\textwidth}
    \vspace{-0.25cm}
     \centering
     \includegraphics[width=0.34\textwidth]{img/real-graphs/dense_split/cora_ml/boxplot_main_x.pdf}
     \caption{(Inductive) Cora-ML. %
     }
     \label{fig:over_robustness_cora_ml}
\end{wrapfigure}
in Appendix \ref{sec:app_boxplot_csbm} shows a similar plot for CSBMs. Results are obtained by applying a
variant of $\ell_2$-weak on a target node $v$. However, as Cora-ML is a multi-class dataset, we ensure all inserted edges connect to the same class $c$, which is different to the class of $v$. The vulnerability of a GCN to adversarial attacks likely stems from the lower quartile of robust node classifications in Figure \ref{fig:over_robustness_cora_ml}. We conjecture \textit{over-robustness} for the upper quartile of highly robust node classifications. In Appendix \ref{sec:app_results_real_world_graphs} we show that combining the GCN with LP significantly reduces the upper extent of its robustness while achieving similar test accuracy and show similar results on other real-world datasets. 



==> Camera Ready Submission_arXiv/chapters/6_related_work.tex <==


We now briefly discuss the most important related work and refer to Appendix \ref{sec:app_related_work} for an extended discussion.
Semantics-aware adversarial robustness was theoretically studied by \citet{revisiting_adv_risk}. Similarly, their work shows no (adversarial) robustness-accuracy tradeoff, postulated among others by \citet{robustness_accuracy_tradeoff}. However, they only discuss i.i.d.\ data and focus on the image domain. A notion of overstability was investigated by \citet{nlp_overstability} in natural language processing. However, their studied perturbations still preserve the ground-truth answers to predict by models. \citet{invariance_based_adv_examples} discussed over-robustness under the name of invariance-based adversarial examples for the image domain. They did not use the concept of a reference classifier, but used humans as a labeling oracle. To the best of our knowledge, we are the first to study a %
notion of over-robustness for graphs, and a robustness-accuracy tradeoff for non-i.i.d.\ data. For graphs, \citet{attack_dai2018} note the possibility of measuring semantics with a gold standard classifier and generate semantic-preserving perturbations for graph classification on Erdős-Rényi graphs. Although no work has explicitly addressed semantic content preservation for node classification, %
\citet{attack_nettack} proposed to approximate unnoticeability by preserving the degree distribution; \citet{attacks_sga} introduced a metric for degree assortativity, but did not restrict perturbations; \citet{attack_gia} proposed a node- and edge-centric homophily metric%
, but focused on adding malicious nodes instead of edges. 


==> Camera Ready Submission_arXiv/chapters/7_discussion.tex <==
We have shown that common threat models on CSBMs include many graphs with changed semantic content. As a result, (full) conventional robustness %
leads to sub-optimal generalization and robustness \textit{beyond} the point of semantic change. But we also found that the same threat models include truly adversarial examples. This dichotomy is caused by the low-degrees of nodes and the brittleness of their class-membership to a few edges. %
Thus, it needs both notions, adversarial and over-robustness for a complete picture of robustness in graph learning. 
As real-world graphs also contain mainly low-degree nodes, this calls for more caution when applying $\ell_0$-norm restricted threat models. These thread models %
should not be an end to, but the start of an investigation into realistic perturbation models and works thinking about unnoticeability are positive directions into this endeavour. On CSBMs a significant part of conventional robustness of GNNs %
is in fact over-robustness (with similar patterns on real-world graphs). This raises the question what kind of robustness do defenses improve on in GNNs? %

Applying label propagation on top of GNN predictions has shown to be a simple way to reduce over-robustness
while not harming generalization or adversarial robustness. Therefore, LP can be seen as a defense against an attack, where the adversary overtakes a clean node (e.g., social media user) and, with its malicious activity, tries to stay undetected. 
This shows that not including the known labels in their predictions can be a significant limitation of GNNs. As visually inspecting graphs is difficult, synthetic graph generation models have proved to be an important tool to further a principled understanding of graph attacks and defenses. %
Concluding, using semantics-aware robustness, we have shown that for inductively classifying a newly sampled node, optimal robustness is achieveable, while maintaining high accuracy. %


==> Camera Ready Submission_arXiv/limitations.tex <==






==> Camera Ready Submission_arXiv/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Camera Ready Submission_arXiv/results_notes.tex <==


\subsection{Attacks}



l2 attack. 




\subsection{Metric} \label{sec:robustness_metric}



Therefore, we measure the relative robustness of a node to its degree and average this measure for all relevant nodes yielding 

\begin{equation}
    \tilde{R}_{f|g} = \frac{1}{|V'|}\sum_{i \in V'}{\frac{\text{Robustness}_{f|g}(i)}{\text{deg}(i)}}
\end{equation}

with $\text{Robustness}_{f|g}(i)$ referring to the robustness of the classification of node $i$ using classifier $f$ measured w.r.t. base classifier $g$. This means that robustness refers to the highest number of edges which can be inserted in the graph until Definition \ref{def:adversarial_perturbation} is violated. $V'$ is referring to the set of inductively added nodes, which (besides being correctly classified) fulfill condition (i) in Definition \ref{def:adversarial_perturbation}.



\subsubsection{Measuring Over-Robustness}








\begin{equation}
    \text{Over-Robustness v2} = 1 - \frac{\tilde{R}_{f|g}}{\tilde{R}_{f}}
\end{equation}



\subsubsection{Measuring Adversarial Robustness}



\begin{equation}
    \text{Adv-Robustness} = \frac{\tilde{R}_{f|g}}{\tilde{R}_{g}}
\end{equation}



\subsection{Over-Robustness of Graph Neural Networks} \label{sec:results_over_robustness}



\subsubsection{Over-Robustness on Real World Graphs}


\subsection{Mitigating Over-Robustness using Label Information} \label{sec:over_robustness_using_label_information}


==> limitations.tex <==






==> results_notes.tex <==


\subsection{Attacks}



l2 attack. 




\subsection{Metric} \label{sec:robustness_metric}



Therefore, we measure the relative robustness of a node to its degree and average this measure for all relevant nodes yielding 

\begin{equation}
    \tilde{R}_{f|g} = \frac{1}{|V'|}\sum_{i \in V'}{\frac{\text{Robustness}_{f|g}(i)}{\text{deg}(i)}}
\end{equation}

with $\text{Robustness}_{f|g}(i)$ referring to the robustness of the classification of node $i$ using classifier $f$ measured w.r.t. base classifier $g$. This means that robustness refers to the highest number of edges which can be inserted in the graph until Definition \ref{def:adversarial_perturbation} is violated. $V'$ is referring to the set of inductively added nodes, which (besides being correctly classified) fulfill condition (i) in Definition \ref{def:adversarial_perturbation}.



\subsubsection{Measuring Over-Robustness}








\begin{equation}
    \text{Over-Robustness v2} = 1 - \frac{\tilde{R}_{f|g}}{\tilde{R}_{f}}
\end{equation}



\subsubsection{Measuring Adversarial Robustness}



\begin{equation}
    \text{Adv-Robustness} = \frac{\tilde{R}_{f|g}}{\tilde{R}_{g}}
\end{equation}



\subsection{Over-Robustness of Graph Neural Networks} \label{sec:results_over_robustness}



\subsubsection{Over-Robustness on Real World Graphs}


\subsection{Mitigating Over-Robustness using Label Information} \label{sec:over_robustness_using_label_information}

